Projective Urban Texturing

This paper proposes a method for automatic generation of textures for 3D city meshes in immersive urban environments. Many recent pipelines capture or synthesize large quantities of city geometry using scanners or procedural modeling pipelines. Such geometry is intricate and realistic, however the generation of photo-realistic textures for such large scenes remains a problem. We propose to generate textures for input target 3D meshes driven by the textural style present in readily available datasets of panoramic photos capturing urban environments. Re-targeting such 2D datasets to 3D geometry is challenging because the underlying shape, size, and layout of the urban structures in the photos do not correspond to the ones in the target meshes. Photos also often have objects (e.g., trees, vehicles) that may not even be present in the target geometry. To address these issues we present a method, called Projective Urban Texturing (PUT), which re-targets textural style from real-world panoramic images to unseen urban meshes. PUT relies on contrastive and adversarial training of a neural architecture designed for unpaired image-to-texture translation. The generated textures are stored in a texture atlas applied to the target 3D mesh geometry. To promote texture consistency, PUT employs an iterative procedure in which texture synthesis is conditioned on previously generated, adjacent textures. We demonstrate both quantitative and qualitative evaluation of the generated textures.

==> content/experiments_old_version.tex <==
\section{Evaluation}
\label{sec:eval}
In this section we evaluate our pipeline on test models generated with the process described in Section \ref{subsec:train_data}.
As discussed earlier, no identical city blocks exist in both our train and test meshes. 
We trained our image translation network separately on the dataset of London and the dataset of New York images according to the procedure described in Section \ref{subsec:training}.
We present qualitative as well as quantitative results.
Qualitative results include both intermediate outputs (generated panoramas)  of our image translation network as well as perspective renderings of our test meshes at street level.
They aim to evaluate our method's ability to generate consistent and plausible textures for an urban mesh, as well as its ability to transfer the distinctive ``style'' of a real city to a virtual one.
Quantitative results include an ablation study of the effects of various parts of our pipeline using the Fr\'echet Inception Distance (FID)\cite{fid_paper}, as well as a user study that aims to perceptually evaluate whether our output textures are more plausible than those generated by the original CycleGAN method \cite{cycleGAN}.

\subsection{Qualitative Evaluation}
First, we evaluate the quality of our method's output textures by placing a perspective camera at street level for each of our test meshes and taking renderings of the meshes textured by our method, pointing the camera towards either side of the street.
Results can be seen in Figure \ref{fig:Style_comparison}, for the networks trained on London and New York data. In addition, we refer readers to the accompanying video showing fly-throughs of $3$ of our London-based test scenes with natural lighting and a procedurally generated sky.
 Our method transfers the appearance of large structures such as multi-storey walls, streets, or sidewalks from real panoramas and is able to often align texture details with geometric ones i.e., texture edges of windows and doors with geometry edges. One `side-effect' of our method is that real-world shadows can also be translated to the streets and sidewalks, as evident in Figure \ref{fig:Style_comparison}.

\paragraph*{City style transfer.} 
% \melinos{need a better title here} 
Our method can be trained on street-level panoramic images collected from different cities in the world, to give urban 3D models the appearance of a city's distinctive style, as illustrated by our London and New York examples in Figure \ref{fig:Style_comparison}.
The generated textured city blocks appear distinctively textured with our pipeline trained on New York versus the ones textured with London panoramas. For example, a red brick-like appearance is visible in the walls of the mesh textured by our network trained in New York panoramas; such appearance is common in New York buildings. On the other hand, meshes textured by our network trained on London panoramas appear with white, yellow and brown distributions of color on their facades, a color distribution which is common around London area. 
%In Figure \ref{fig:3D_facade_comp} we observe the different styles between London and New-York, and verify the color and style of generated panoramas match different distributions based on the city that it was trained on. 
We provide additional comparisons showing real-world panoramas and panoramic images rendered from our textured city blocks from London and New York in Figures \ref{fig:real_fake_comparison} and \ref{fig:real_fake_comparison_NY}. We can observe that the generated outputs follow color  distributions of given cities. Looking at the real-world panoramas, we observe the differences between the two cities: New York's facades often consist of gray-red shades of colors while London' facades tend to be brighter with yellow to blown color distributions. These distributions  are also encountered in our generated textures.

%Results section contains visual and quantitative results comparing different models and texture styles from different cities. For the visual evaluation we use the model with the highest FID score. Models were train based on London panoramic images data-set for all evaluation sections except of subsection \ref{subsec:CityMesh} where we fine-tune generators on Nicosia and New-York data-sets that was trained on New-York panoramic images. For the experiments the interpolation between frames on texturing pipeline is set to $0.75$.
%\subsection{3D Textured City Mesh}
%Figure \ref{fig:london_mesh} illustrate our final goal result to generate realistic textures for 3D meshes. Extracted figures \ref{fig:london_mesh_1} and \ref{fig:london_mesh_2} show how the rendering is close to London color and style distribution. Additionally we observe diversity of styles on building that our generator fitted building structures on different styles distributions based on height, window shapes, and floor number. Interestingly the generator respects the geometry of the 3D City Mesh and shapes its output to fit windows, doors and other facade artifacts on the correct areas.
% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/render_LO1_gimp.png}
        
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/render_NY1_gimp.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/render_LO2.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/render_NY2.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/render_LO3.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/render_NY3.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/comparison_figure_London.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/comparison_figure_NY.png}
%     \end{subfigure}
%     \caption{Renderings of a test mesh textured by our method trained on London (left) and New York (right) panoramas. We show street-level (top three rows) and orthographic (bottom row) viewpoints.}
%     \label{fig:Style_comparison}
% \end{figure*}

% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/render_NY1.png}
%         \caption{}
%         \label{fig:NY_mesh_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/render_ny2.png}
%         \caption{}
%         \label{fig:NY_mesh_2}
%     \end{subfigure}
%     \caption{Street-level renderings of a test mesh textured by our method trained on London and New York panoramas. \melinos{include more}}
%     \label{fig:NY_mesh}
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}[b]{0.5\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/real_london_510.jpg}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{0.5\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/real_london2.jpg}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.5\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/00510.png}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{0.5\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/00508.png}
%     \end{subfigure}
%     \caption{Comparison of real photographs (top) and generated images from our network (bottom) for London.}
%     \label{fig:real_fake_comparison}
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}[b]{0.5\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/real_NY1.jpg}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{0.5\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/real_NY2.jpg}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.5\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/fake_NY1.png}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{0.5\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/fakeNY2.png}
%     \end{subfigure}
%     \caption{Comparison of real photographs (top) and generated images from our network (bottom) for New York.
%     % This figure show the correlation of 2D and 3D outputs. Images on bottom resulted on the textures for the facades of the 3D meshes on top.
%     }
%     \label{fig:real_fake_comparison_NY}
% \end{figure}


% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=1\columnwidth]{imgs/frank.png}
%     \caption{}
%     \label{fig:frank}
% \end{figure}

%\subsubsection{FID Scores}

%\subsubsection{3D City Mesh and 2D panorama Correspondence}
%As camera moves on a predefined path, it renders a panoramic image of the mesh considering an intermediate UV mesh. Then the generator converts gray geometry to realistic image. Thus, as a result we got a sequence of panoramic image which are being projected on the 3D mesh. Figure \ref{fig:london_galery} display the 2D and 3D perspective of our outputs.

% Figure: 3x 3D renders of the different city meshes.

% Figure: 3 x 3 table of cells ( 3 x different styles ) x (3 x different mesh-sources). Perhaps 2x panoramas per table cell.


%\subsubsection{Different City/Style Generation}\label{subsec:CityMesh}
%We test the applicability of our approach on different styles from different cities. In figure \ref{fig:3D_mesh_comparisson} we display 3D rendering from the same 3D scene textured in 2 different styles. London and New-York differ in terms of style,for New-York meshes we tend to generate red and black distribution of facades while London meshes facade distributions tend to be between white and brown colors. 
% Figure: Example panoramas from each of the 3 cities GT (which look like generated examples).


\paragraph*{Consistency.}
% \melinos{why just six}\yiangos{base on the facade length it needs the corresponding number of panos, we can show more or less panos it make no difference}
We qualitatively evaluate the degree of consistency between consecutive output textures from our architecture 
in Figure~\ref{fig:london_galery}. We display six  consecutive intermediate panoramic outputs of our image translation network trained on the London dataset. We note that consecutive outputs appear to be consistent in accordance to previous ones. 
This helps to preserve details in the generated texture maps, as seen at the top of Figure
\ref{fig:london_galery} which shows a close-up rendering of textured 3D meshes on both sides of the street.
Figure \ref{fig:consistency} also shows how partially textured images are translated into fully textured ones, helping with the  consistency of the generated texture. The overall appearance of the already textured part of the mesh smoothly blends with the untextured parts.
%\melinos{not sure about this image and what we are trying to show - maybe merge to \ref{fig:london_galery} ? and make that one larger by showing both final (output) and input panoramas?}. 

% \begin{figure}[!ht]
%     \includegraphics[width=\columnwidth]{imgs/LO_gallery_both_sides.pdf}
%     \caption{Top: renderings of textured buildings on opposite sides of a street, in a test mesh textured by our network trained on London panoramas. Bottom: six of the generated network outputs used to texture the above buildings. Note that both buildings exist in the panoramic outputs.}
%     \label{fig:london_galery}
% \end{figure}


% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/figure_11_32.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/figure_11_64.png}
%     \end{subfigure}
%     \caption{Left column: partially textured images used as input to our image translation network $g$. Right column: resulting network outputs. The output image appears to be consistent with both the partial textures and geometry.}
    %\caption{Consistency outputs given previously generated texture.example inputs and outputs for a variety of GT consistency images, geometry, and masks. (How about ?: center left is one example showing inputs and outputs. above right: 2xdifferent mask + output. middle right: 2x different consistency and outputs. bottom right: 2xdifferent geometry and outputs.}
    % \label{fig:consistency}
% \end{figure}

\paragraph*{Comparisons with the original CycleGAN.}
Figure \ref{fig:cycle_fail} (top) shows results of the original CycleGAN method: the method was trained on London data to learn the mapping between the domain of grayscale renderings and real-world panoramas directly i.e., without using partial textured images, and without the inter-frame consistency loss. We observe that
 consecutive panoramas often differ due to tree artifacts suddenly appearing in the second and third panorama. The color of the facade in the fourth panorama differs from the first generated panorama. On the other hand, our network generates panoramas in a more consistent manner \ref{fig:cycle_fail} (bottom).
Figure \ref{fig:3D_facade_comp} shows differences of the original CycleGAN and our method in the output textured buildings, after applying our texture propagation step for both methods. Half of the textured building generated by the original CycleGAN has green-like appearance (e.g., grass- or tree-texture), which makes it inconsistent with the other half. In contrast, our textured building has a more consistent appearance. 

% \begin{figure*}[!h]
%     \centering
%      \begin{subfigure}[b]{2\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{imgs/cycle_gan_fail1.png}
%         \label{fig:consistency_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{2\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/figure13_consistent.jpg}
%         \label{fig:consistency_2}
%     \end{subfigure}
%     \caption{Panoramic images generated by CycleGAN (top) and \name (bottom) for the same geometry. Note that \Name improves consistency over the building color and texture.}
%     \label{fig:cycle_fail}
% \end{figure*}


% \begin{figure}[!h]
%     \centering
%      \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{imgs/facade3_Base.png}
%         \label{}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{imgs/facade3_Con.png}
%         \label{}
%     \end{subfigure}
%      \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{imgs/facade7_Base.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{imgs/facade7_Con.png}
%     \end{subfigure}
%     \caption{Results of applying texture propagation to CycleGAN (left) and \name (right) panoramic network outputs. Note that \Name yields a more consistent style over the facade.}
%     \label{fig:3D_facade_comp}
% \end{figure}

\subsection{Quantitative Evaluation}

% sets: real, synthetic textured, synthetic geometry, cycleGAN outputs, cycle-ESRGAN  outputs, blendNet outputs, our 3D model rendered from a "novel" viewpoint, google earth, frankenGAN mesh.
%In lack of a suitably similar method to compare our method against, we choose to compare to a original CycleGAN version of our method without consistency loss and without merged inputs using an ablation study as well as a user study.
Here we discuss our ablation study that numerically evaluates technical choices for our method. We continue to present a user study that compares our method with the original CycleGAN.

\paragraph*{Ablation Study.}
For the ablation study we rely on the The Fr\'echet Inception Distance~\cite{fid_paper}.
%Fr\'echet Inception Distance (FID).
 FID is a measure of the distance between feature vectors extracted from real and generated images. Low scores indicate that feature statistics in the generated images agree more with ones in real images.
%For the experiment we use 976 geometry panorama test samples and 5000 real panoramas from London area. 
Table \ref{tab:ablation_study} reports FID scores for three variants of \name. The first variant, \nameA, is trained an image translation network without the inter-frame consistency loss. It uses only the adversarial and the cycle consistency losses, as in the original CycleGAN approach. The second variant, \nameB, renders a grayscale image of the 3D geometry separately from the partial textured rendering, then concatenates the two images channel-wise, yielding a 4-channel image. The network of this variant is trained to process this 4-channel image with all losses (including the inter-frame consistency loss).
The last model, \nameC, is our full method using all losses and processes a single RGB image containing both grayscale and partially textured areas.
 Based on the FID results, we observe that our full method outperforms the above first two reduced variants. Using a single RGB image seems to help the network blend textured and untextured parts. The inter-frame consistency loss also has a positive impact on the FID score. 
 %Treating the grayscale image as an extra channel seems to increase the difficulty for the network to blend the textured and untextured parts
 % \name3 outperforms all the other models and illustrate the contribution of consistency loss for this task.

% \begin{table}[h!]
%   \begin{center}
%     \caption{Ablation study FID scores.}
%     \label{tab:ablation_study}
%     \begin{tabular}{||@{}c@{}|c|c|c|c|c||}
%     \hline
%       \textbf{Model} & \textbf{Consistency Loss} & \textbf{RGB input} & \textbf{FID}$\downarrow$\\
%       \hline\hline
%       \nameA  & \textendash & \checkmark & 72.711 \\
%       \nameB  & \checkmark & \textendash & 80.329 \\
%       \nameC  & \checkmark & \checkmark & \textbf{65.250} \\
%       \hline
%     \end{tabular}
%   \end{center}
% \end{table}

\begin{table}[h!]
  \begin{center}
    \caption{\yiangos{CHANGED!} Ablation study FID scores.}
    \label{tab:ablation_study}
    \begin{tabular}{||@{}c@{}|c|c|c|c|c||}
    \hline
      \textbf{Model} & \textbf{Consistency Loss} & \textbf{RGB input} & \textbf{FID}$\downarrow$\\
      \hline\hline
      \nameA  & \textendash & \checkmark & 49.732 \\
      \nameB  & \checkmark & \textendash & 43.979 \\
      \nameC  & \checkmark & \checkmark & \textbf{43.371} \\
      \hline
    \end{tabular}
  \end{center}
\end{table}

Figure \ref{fig:ablation_study_visual} shows comparisons of these variants.  \nameA seems to often generate inconsistent texture within the same building structure (as we also observed in the original CycleGAN). \nameB seems to have trouble creating coherent textures. Visible artifacts, or seams, are more common in \nameA and \nameB, rather than \nameC.
 %Visual results is coherent with \ref{tab:ablation_study} regrading \name2 as it provides the worst results even though it keeps the previous textures constant. We spot several tree-like artifacts around the buildings, the blending between textured and untextured parts is less noticeable than \name1 in this case. \name3 use 3-channel input and a consistency loss, givre the outputs we conclude that it respects previous textures and tries to generate similar styles, moreover the boundaries between textured and untextured parts are less obvious. The superiority of \name3 is verified by both FID and visual comparison results.  

% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/00079.png}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/00242.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/00886.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/01025.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/00900.png}
%     \end{subfigure}
%     \caption{Comparison between \name variations (as in Table~\ref{tab:ablation_study}). The first, second, and third column show results from \nameA, \nameB, \nameC respectively. The rows have identical underlying 3D geometry.}
%     \label{fig:ablation_study_visual}
% \end{figure}
% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/methodology/00107.png}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/methodology/00974.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/methodology/00111.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/methodology/00124.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{1\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{imgs/methodology/00411.png}
%     \end{subfigure}
%     \caption{\yiangos{CHANGED!}Comparison between \name variations (as in Table~\ref{tab:ablation_study}). The first, second, and third column show results from \nameA, \nameB, \nameC respectively. The rows have identical underlying 3D geometry.}
%     \label{fig:ablation_study_visual}
% \end{figure}

% \begin{table*}[h!]
%   \begin{center}
%     \caption{Consistency Generator ablation study.}
%     \label{tab:ablation_study}
%     \begin{tabular}{||c|c|c|c|c|c|c||}
%     \hline
%       \textbf{Model} & \textbf{Consistency Loss} & \textbf{Merge Inputs} & \textbf{Mask Dilation for consistency loss} & \textbf{FID}$\downarrow$ & \textbf{FID*}$\downarrow$\\
%       \hline\hline
%       Baseline & \textendash & \textendash &  \textendash & 55.994 & - \\
%       \name 1  & \textendash & \checkmark  & \textendash & 62.728 & 72.711 \\
%       \name 2  & \checkmark & \textendash & \textendash & 57.032 & 73.663 \\
%       \name 3  & \checkmark & \checkmark & \textendash & \textbf{55.824} & 71.379 \\
%       \name 4  & \checkmark & \textendash & \checkmark & 61.435 & 80.329 \\
%       \name 5  & \checkmark & \checkmark & \checkmark & 58.707 & \textbf{65.250} \\
%       \hline
%     \end{tabular}
%   \end{center}
% \end{table*}

\paragraph*{User study.}
Our user study aimed to perform a perceptual evaluation of the results of our method versus the original CycleGAN approach \cite{cycleGAN}.  To execute our user study, 
 we assembled a pool of $10$ webpages per questionnaire. Each page showed two images: one image showed a rendering of a city block textured with the original CycleGAN, and the other image showed the rendering of the same block textured with \name (Figure \ref{fig:user_study}).
 The two images were placed in randomly picked left/right positions for each webpage.
 Each webpage included the following question:
 ``Which of the two synthetic images has less artifacts and appears more plausible?''
 The study was executed on the Mechanical Turk (MTurk) platform. 
The MTurk participants were asked to pick one of the following choices: ``left image'', ``right image'', ``can't tell - both are equally plausible'',  ``can't tell - none are plausible''.  
Each MTurk participant was asked to complete a questionnaire with $20$ queries (webpages) randomly picked from our pool. Pages were shown in a random order. Each query was repeated twice (i.e., we had $10$ unique pages per questionnaire), with the two renderings randomly flipped each time to detect unreliable participants giving inconsistent answers. 
 We filtered out unreliable MTurk participants who gave two different answers to more than $5$ out of the $10$ unique queries in the questionnaire, or took less than a minute to complete it.
Each participant was allowed to answer only a single questionnaire to ensure participant diversity. 
We had $25$ different, reliable MTurk participants.
Each MTurk participant voted for $10$ unique queries twice. We kept only the persistent votes i.e., votes that were the same for both repetitions of the query (out of $250$ votes, $195$ were persistent). 
\name received $111$ persistent votes ($56.9\%$) versus the original CycleGAN that received $64$ votes ($32.8\%$). The answer ``both are equally plausible'' got $5$ votes ($2.6\%$), and the answer ``none are plausible'' got $15$ votes ($7.8\%$).
Based on these results, we observe that the majority of MTurkers selected \Name as the more plausible image considerably more frequently than the original CycleGAN.  

% \begin{figure}[!h]
%     \centering
%         \includegraphics[width=1\columnwidth]{imgs/user_study.png}
%         \caption{Screenshot from  our user study interface. In this screenshot, the left image is produced by \name, and the right image is produced by the original CycleGAN.}
%         \label{fig:user_study}
% \end{figure}

\paragraph*{Computation and memory requirements.} We trained our model for approximately $7$ days on
 $4$ NVIDIA Tesla M40 graphics cards. Each epoch requires $1.75$ hours to complete. The forward pass for the image translation network takes $12.1$ ms per panorama output at test time. 
 %For the \name pipeline the size of the scene, the number of the frames and the resolution on the UV image determine the time that the texturing is gonna take.
 To perform one iteration of our pipeline, including rendering, forward pass through the translation network, and texture propagation to a a $6114$x$6114$ atlas requires $44$ seconds. Creating the whole texture atlas for the largest mesh in our tests takes approximately $30$ minutes.
 The required system (CPU) memory is $15$ GB of RAM for the largest mesh in our tests.  %based on the size of the testing scene.

==> content/related_city.tex <==
%tom

% https://github.com/ZPdesu/lsaa-dataset

Virtual urban environments have become ubiquitous for city planning, video game environments, and mapping. Following this trend there are increasing numbers of 3D city model sources - both for reconstruction of existing environments and \emph{synthesis} of planned or fictional cityscapes. The reconstruction of existing environments~\cite{musialski2013survey}, using techniques such as photogrammetry~\cite{baillard1999automatic,zhu2018large}, capture meshes with textures. Therefore, we concern ourselves here with synthesised meshes; these have the advantage of being able to represent urban environments that are being planned, fictional, or simulated.

%\textbf{Reconstruction techniques} approximate the city-as-built from observations. We discuss highlights here and refer the reader to summaries from the graphics~\cite{musialski2013survey} and remote sensing~\cite{haala2010update} communities for additional depth. Reconstruction from 2D \emph{cartographic data} sources is simple, but limited. Typical pipelines simply extrude building footprints~\cite{haala19983d} and create a roof~\cite{laycock2003automatically} , although modern cartographic standards such as CityGML~\cite{groger2012citygml, biljecki2016improved} are rapidly developing more nuance. With modern Geographic Information Systems (GIS) it is possible to create huge 3D urban meshes with these approaches~\cite{biljecki2017generating}, although mostly untextured. \emph{Point clouds} (typically from Lidar or structure-from-motion systems) are converted to 3D mesh representations using techniques such as Poisson reconstruction~\cite{Kazhdan2006,kazhdan2013screened}, planar patch identification and fusion~\cite{monszpart2015rapter, lafarge2012creating, fang2020connect}, or semantic segmentation~\cite{lin2013semantic}. Reconstruction approaches vary - large area aerial Lidar showing only roof heights~\cite{lafarge2010structural}, require different approaches to dense, street-side Lidar, capturing detailed facades~\cite{brenner2016scalable} \melinos{not sure this parses}. \emph{Photogrammetry} can be used to recover 3D information from aerial~\cite{baillard1999automatic,zhu2018large} and street level geometry~\cite{teller1998automated, snavely2006photo}\melinos{you mean photography?}. Various models have been used to fit meshes to raw images, including procedural~\cite{teboul2013parsing, nishida2018procedural}, unwrappable~\cite{fang2013image}, Markovian~\cite{kozinski2015mrf}, or deep~\cite{femiani2018facade} models to facade images. 

%The popularity of photography has created large data-sets which we process to create.


%Towards large-scale city reconstruction from satellites
%Coupling a panoramic camera with a global positioning system (GPS) and 
% https://perso.telecom-paristech.fr/boubek/papers/GeoPrimFitSurvey/comparison-webapp/index.html
%Paris looks like paris~\cite{doersch2012makes}


%Fusing \emph{multiple data sources} significantly increases complexity of the algorithms used, but is able to combine features from different sources. Early examples involved projecting panoramic images on GIS meshes~\cite{teller1998automated}. More recently typical pipelines build a core parametric or procedural representation with contributions from aerial data for large scale and roof features or street-level data for facade features. For example, Zeng et al.~\cite{zeng2018neural} fit procedural models to Lidar data before augmenting with roof features from satellite photos. Similarly, Kelly et al.~\shortcite{kelly2017bigsur} simultaneously combine photogrammetric meshes, GIS footprints, and street level photos to build a parametric model based on Procedural Extrusions~\cite{kelly2011interactive}. However, these approaches do not generate facade textures.

% Synthesis approaches to 3D city models are manually authored~\cite{vanegas2010modelling}. 

Synthesis of urban geometry may be manual or procedural. In a manual pipeline designers will build meshes using specialised software from scratch~\cite{lipp2014pushpull++} or guided by images~\cite{nan2010smartboxes}. Such manual approaches can be slow for massive urban areas. A faster approach is procedural modeling using languages such as Split Grammars~\cite{wonka2003instant, Mueller:2006:PMB} or Procedural Extrusions~\cite{kelly2011interactive} -- these models can be driven by various goals such as optimisation~\cite{Schwarz:2015:APM}, inverse procedural modeling~\cite{Wu:2014:IPM, Martinovic:2013:BGL}, or directly from real world data~\cite{kelly2018frankengan}. The grammars and programming languages used to procedurally generate cityscapes have typically focused on the generation of geometry -- texturing has typically been an afterthought. Synthesised urban meshes have a wide variety of characteristics due to the variety of goals, approaches, data (resolution, accuracy, and range), and techniques (aerial, street-side, procedural, vehicle-mounted).

%fixme: following doesn't flow into next section
%Several attempts have been made to create image based tools~\cite{muller2007image} to create procedural texture-rules for urban environments. However these are problematic due to the over-compartmentalisation or lack of context in grammars such as CGAShape; adjacent faces (e.g. walls) are not aware of their neighbours and so cannot respond (e.g. brick textures are not aligned around building corners). In this paper we will demonstrate the joint texturing of urban surfaces to address this issue.


%Hybrid approach with geometry~\cite{debevec1996modeling}  
%facade wizard ~\cite{muller2007image}}



==> content/related_textures.tex <==

Textures are an essential component of modeling urban appearances; they add visual information about material as well as a low-cost approximation of geometric information ~\cite{gruber1995geometric}.
%
To texture reconstructed geometry, directly projecting photographs onto geometry~\cite{niem1995mapping, bohm2004multi,bornik2001high} produces high quality results, but has several disadvantages: it requires exact photo locations (i.e. noise-free location data~\cite{klingner2013street}), the images must be unobstructed (e.g. occlusions by trees or vehicles~\cite{FanCompletion}), and the geometry consistent with the photographs. 
%
Further, this approach isn't applicable to synthesis pipelines. In these situations we are concerned with urban texture \emph{synthesis}.

\textbf{Texture synthesis} is the generation of texture images from exemplars or lower dimension representations.
%has recently rapidly given way to image synthesis as deep architectures are applied to the problem of the creation of materials. 
Traditional learning-based methods generate textures with local and stationary properties, using techniques such as Markov Random Fields to generate pixels~\cite{efros1999texture,WeiTree} or patches~\cite{LiangPatch, efros2001image} from an exemplar image. Variations on these themes generate larger, more varied, textures fast~\cite{darabi2012image}. Procedural languages to create textures~\cite{muller2007image} are well adapted for urban domains. However, much of the realism of urban scenes is due to the heterogeneous appearance of surfaces due to weathering and damage. Approaches to model these phenomena include L-Systems for rust~\cite{chang2003synthesis}, $\gamma$-ton tracing for weathering and aging~\cite{chen2005visual, PE:VMV:VMV12:063-070}, or more general context-aware~\cite{lu2007context} textures to transfer appearance.
%See Wei et al.~\cite{SynthesisPauly} for an overview. % << delete
With the advent of Convolutional Neural Networks (CNNs), example-based texture synthesis has increasingly become a data-driven process, creating textures by gradient descent in feature space~\cite{gatys2015texture} or with GANs~\cite{ZhouTextureSynthesis,fruhstuck2019tilegan}. Another approach to texture generation is to transform an input image to a different style or domain. Such image-to-image translation~\cite{pix2pix} may disentangle the structure from the style to enable style transfer~\cite{gatys2016image}. These have been applied to generate terrains~\cite{guerin2017interactive} and chained sequences~\cite{kelly2018frankengan} for urban-domain specific texture pipelines.
Several projects have explored learning~\cite{sharma2019unsupervised} from and completion~\cite{song2018im2pano3d} of panoramic images using neural networks.

Where there are no datasets of paired input and output images, \emph{unsupervised} image-to-image networks use novel losses to generate images and textures. A typical approach is to use a cycle loss~\cite{cycleGAN} which learns to translate from one image domain to a second, and also from the second to the first. This reconstruction loss is applied alongside other losses, such as adversarial loss, for unsupervised texture learning. This technique has been extended to multi- domain~\cite{choi2018stargan,huang2018multimodal}, patches~\cite{CUT}, and domain specific problems such as urban image~\cite{guo2019gan} and video generation~\cite{ wang2018video}.

%These techniques account for the 3D manifold, beyond planar images - at the corners of a building, a good texture will wrap seamlessly.  To ensure that textures wrap correctly around the corners of buildings requires the texturing of a 2D manifold embedded in 3D space. 

\textbf{3D Textures} presents several challenges. Synthesising 3D details~\cite{WhitingMasonry, CutlerSolid} with detailed volumetric information is expensive. If we do not require information inside the mesh, such effects can be created at lower cost by taking a ``thick-skin'' approach~\cite{LegakisCellular}. To neurally generate a seamless texture over a large 3D mesh we might use 3D CNNs to generate voxel colours~\cite{oechsle2019texture} as well as geometry~\cite{wu2016learning, wen2019pixel2mesh++}, however the high memory requirement limits the output resolution and the lack of volumetric texture datasets is also problematic. Attempts to overcome these limitations are ongoing, using polygon-based~\cite{kato2018neural}, 3D noise~\cite{henzler2020neuraltexture}, and point-based renderer~\cite{meshry2019neural} approaches; results are generally low resolution or only in screen-space. For these reasons, neural texturing systems seem most effective over a 2D manifold, as it allows them to apply any of the above 2D texture generation techniques. Our method learns over the 2D image space, using an existing 2D texture generation technique~\cite{CUT}, together with a blending approach to wrap the texture over the manifold.

Early \textbf{texture blending or 2D inpainting} systems typically match small image patches~\cite{LiangPatch, efros2001image}, or minimize a function over a grid of pixels using column / row energy minimization~\cite{seamCarvingResize} and over arbitrary shapes using graph cuts~\cite{kwatra2003graphcut, rother2004grabcut}, or Poisson~\cite{perez2003poisson} formulations. Although such local approaches produce excellent pixel-level results, they do not contain the higher level knowledge to blend textures and images with more structure. We may overcome this limitation with user input~\cite{agarwala2004interactive} or augmenting our images with labels~\cite{HaysSceneCompletion}; however, recent neural architectures~\cite{zhan2019spatial,zhang2020deep} have improved on the results of these hand-crafted heuristics using techniques such as guided Poisson constraints~\cite{wu2019gp}, symmetry~\cite{deng2018uv}, and searching for latent encoding of compatible adjacent images~\cite{fruhstuck2019tilegan}.

\textbf{Texture combination over 3D objects} combines multiple semi-accurate 2D images or exemplars over a 3D manifold, for example by projection~\cite{pulli1997view, buehler2001unstructured}. These techniques have been applied to a number of domains including 3D photography~\cite{hedman2017casual}, structure-from-motion reconstruction~\cite{kniaz2018thermal}, and video stabilisation~\cite{kopf2014first}. To complete the textures, missing areas are synthesised, frequently using warping~\cite{chaurasia2013depth}, CNNs~\cite{hedman2018deep}, neural renderers~\cite{Raj_2019_CVPR_Workshops}, or GANs~\cite{huang2020adversarial} for blending. 

%Unsupervised texture transfer from images to model collections~\cite{wang2016unsupervised}
% \subsection{Panoramic Images} \twak{moved to introductino}
% Panoramic images have become a cheap and fast way to capture texture information about our urban environments~\cite{anguelov2010google}. Advances in optics have allowed us to create 360 degree panoramas which are well suited to capturing omni-directional information about cities - particularly at street level where a single panoramic image captures opposing facades, overhanging features (bridges and trees), and the street itself. Panoramic image sensors are now commodities including models such as the \emph{Insta360 One X}. Because the images are 2D, a wide corpus of neural learning techniques are available to use.



